Book free $3$-Uniform Hypergraphs

A $k$-book in a hypergraph consists of $k$ Berge triangles sharing a common edge. In this paper we prove that the number of the hyperedges in a $k$-book-free 3-uniform hypergraph on $n$ vertices is at most $\frac{n^2}{8}(1+o(1))$.

==> backup.tex <==
Let us start with the special case of $2$-books,i.e. diamond free hypergraphs.
\begin{lemma}
\label{diamond}
For a $3$-uniform diamond free hypergraph $H$ on $n$ vertices, $e(H)\leq \dfrac{n^2}{8}(1+o(1))$. 
\end{lemma}
\begin{proof}
    %Note that in $G$ we are left with just some triangles or edges, which are hyperedges and some $2$-edges in the original hypergraph $H$.  We claim that $G$ does not have have more than $3$ triangles sitting on an edge.  Say there is an edge which has $4$ triangles sitting on it.  There are few cases to deal with.
    
    %Note that $H'$ is a $2-3$uniform hypergraph.  
    We claim that $G$ does not have have more than $3$ edges sharing a pair of vertices.  Let $u, v$ be a pair of vertices that is contained in $4$ hyperedges, namely $uvx_i$, where $1\leq i \leq 4$.  Without loss of generality, we can assume that the edges $ux_i$ are colored blue and  denote the vertex of the hyperedge sitting $ux_i$ with $y_i$.  There are few cases to deal with, which are as follows:
    \begin{enumerate}
        \item Case $1$: The hyperedges sitting on the edge $ux_i$ are distinct.  It is easy to see that the diamond $ux_1vx_2$ is formed by hyperedges $ux_1y_1, uvx_1,uvx_3, uvx_2$ and $ux_2y_2$ respectively.  

        \item Case $2$: The hyperedges sitting on any two $ux_i$ are same.  Without loss of generality, lets assume $ux_2x_1$ is the given hyperedge.  The hyperedges $uvx_3, uvx_1$ and $ux_1x_2$ constitute a triangle $uvx_1$.  The other two edges of the diamond is formed by hyperedges $ux_4y_4$ and $uvx_4$. 
    \end{enumerate}
    
    %\begin{enumerate}
     %   \item The vertices $y_1$ and $y_2$ are disjoint from each other and $x_i$'s  (see Figure \ref{$4$ triangles on an edge} a).  It is easy to see $ux_1vx_2$ form the vertices of a diamond.
      %  \item Any two of the triangles sitting on the edge $ux_1, ux_2$ and $ux_3$ can share the third vertex, which is different from $x_i$'s.  
      % \item Any two of the triangles sitting on the edge $ux_1, ux_2$ and $ux_3$ can share the third vertex, which is one of the $x_i$'s.
    %\end{enumerate}
    Thus each edge in $G$ is in at-most $3$ triangles.  Thus the structure we are left with wheel like structure as in the following Figure.  We can delete the alternate triangles, as its linear in number, to get a linear hypergraph.  We claim this linear hypergraph is triangle free.  Denote the vertices of hyperedges with $v_i$'s, see Figure \ref{diamond_triangle_free}.  Say we add a triangle $v_1v_3v_5$ by adding the hyperedge $v_4v_5v_6$.  We immediately get another triangle sitting on the edge $v_3v_5$ by the hyperedges $v_3v_5v_6$ and $v_5v_6v_7$.  
    \begin{claim}
    We can delete $9k$ hyperedges from the linear hypergraph to get a triangle free hypergraph.
    \end{claim}
    \begin{proof}
    Consider a hyperedge formed by the vertices $x,y$ and $z$.  Let $S_{x,y}=\{v_i\mid xyv_i \text{ forms a berge triangle}\}$. Note that $|S_{x,y}|\leq 3k$.  Similarly we can bound $S_{y,z}$ and $S_{x,z}$.  Deleting these $9k$ hyperedges leaves us with a triangle free linear hypergraph. 
    \end{proof}
    We also know the maximum number of hyperedges in a triangle free linear hypergraph is $\dfrac{n^{2}}{8}$ \cite{gyori1}. Hence we are done.
    
\begin{figure}[h]
    \centering
    \begin{tikzpicture}[scale=0.35]
    \draw[fill=black](0,0)circle(3pt);
    \draw[fill=black](0,3)circle(3pt);
    \draw[fill=black](-3,0)circle(3pt);
    \draw[fill=black](-3,-3)circle(3pt);
    \draw[fill=black](0,-3)circle(3pt);
    \draw[fill=black](3,3)circle(3pt);
    \draw[fill=black](3,0)circle(3pt);
    \draw[fill=black](3,-3)circle(3pt);
    \draw[fill=black](6,0)circle(3pt);
    \node at (1,-1){$v_1$};
    \node at (1,4){$v_9$};
    \node at (-4,1){$v_8$};
    \node at (-4,-4){$v_2$};
    \node at (1,-4){$v_3$};
    \node at (4,4){$v_4$};
    \node at (4,1){$v_5$};
    \node at (4,-4){$v_6$};
    \node at (7,1){$v_7$};
    
    \draw[black, thick](0,0)--(-3,0)--(0,3)--(0,0)--(-3,-3)--(0,-3)--(0,0);
    \draw[black, thick](0,0)--(3,3)--(3,0)--(6,0)--(3,-3)--(3,0)--(0,0);
    \draw[red, thick](3,-3)--(0,-3)--(3,0);
    \end{tikzpicture}
    \caption{The three linear hypergraph, where red edges denote the new hyperedge being added to form a triangle.}
    \label{diamond_triangle_free}
\end{figure}
\end{proof}

\begin{figure}[h]
\centering
\begin{tikzpicture}[scale=0.25]
\draw[fill=black](-6,0)circle(3pt);
\draw[fill=black](6,0)circle(3pt);
\draw[fill=black](0,6)circle(3pt);
\draw[fill=black](0,-6)circle(3pt);
\draw[fill=black](0,12)circle(3pt);
\draw[fill=black](0,3)circle(3pt);
\draw[fill=black](-6,6)circle(3pt);
\draw[fill=black](-6,-6)circle(3pt);
\node at (-7,-1){$u$};
\node at (0,-7){$x_3$};
\node at (6,-1){$v$};
\node at (0,2){$y_1$};
\node at (0,7){$x_1$};
\node at (0,13){$x_2$};
\node at (-7,6){$y_2$};
\node at (-7,-6){$y_3$};
\draw[blue, thick](-6,0)--(6,0);
\draw[blue, thick](-6,0)--(0,6);
\draw[blue, thick](-6,0)--(0,3);
\draw[blue, thick](-6,6)--(0,12);
\draw[blue, thick](-6,0)--(0,12);
\draw[blue, thick](-6,0)--(0,-6);
\draw[blue, thick](-6,0)--(-6,-6);
\draw[red, thick](0,6)--(6,0);
\draw[red, thick](0,12)--(6,0);
\draw[red, thick](-6,6)--(-6,0);
\draw[red, thick](-6,-6)--(0,-6);
\draw[red, thick](0,-6)--(6,0);
\draw[red, thick](0,6)--(0,3);
%\caption{All the $y_i's$ are distinct.}
\end{tikzpicture}
\begin{tikzpicture}[scale=0.25]
\draw[fill=black](-6,0)circle(3pt);
\draw[fill=black](6,0)circle(3pt);
\draw[fill=black](0,6)circle(3pt);
\draw[fill=black](0,-6)circle(3pt);
\draw[fill=black](0,12)circle(3pt);
\draw[fill=black](0,9)circle(3pt);

%\draw[fill=black](-6,6)circle(3pt);
\node at (-7,-1){$u$};
\node at (0,-7){$x_3$};
\node at (6,-1){$v$};
\node at (-1,8){$y_1$};
\node at (0,7){$x_1$};
\node at (0,13){$x_2$};
\node at (-7,-6){$y_3$};
\draw[fill=black](-6,-6)circle(3pt);
%\node at (-7,6){$y_2$};
\draw[blue, thick](-6,0)--(-6,-6);
\draw[blue, thick](-6,0)--(0,-6);
\draw[blue, thick](-6,0)--(0,6);
\draw[blue, thick](-6,0)--(0,9);
\draw[blue, thick](-6,0)--(0,12);
\draw[blue, thick](-6,0)--(6,0);
\draw[red, thick](0,12)--(6,0);
\draw[red, thick](0,6)--(6,0);
\draw[red, thick](0,-6)--(6,0);
\draw[red, thick](-6,-6)--(0,-6);
\draw[red, thick](0,12)--(0,6);
%\caption{Two of the $y_i$'s are distinct.}
\end{tikzpicture}

\begin{tikzpicture}[scale=0.25]
\draw[fill=black](-6,0)circle(3pt);
\draw[fill=black](6,0)circle(3pt);
\draw[fill=black](0,6)circle(3pt);
\draw[fill=black](0,-6)circle(3pt);
\draw[fill=black](0,12)circle(3pt);
\draw[fill=black](0,18)circle(3pt);
\draw[fill=black](-6,12)circle(3pt);
%\draw[fill=black](0,9)circle(3pt);

%\draw[fill=black](-6,6)circle(3pt);
\node at (-7,-1){$u$};
\node at (0,-7){$x_3$};
\node at (6,-1){$v$};
%\node at (-1,8){$y_1$};
\node at (0,7){$x_1$};
\node at (0,13){$x_2$};
\node at (-7,-6){$y_3$};
\node at (0,19){$x_4$};
\node at (-7,12){$y_4$};
\draw[fill=black](-6,-6)circle(3pt);
%\node at (-7,6){$y_2$};
\draw[red, thick](0,12)--(6,0);
\draw[red, thick](0,6)--(6,0);
\draw[red, thick](0,6)--(0,12);
\draw[red, thick](0,-6)--(6,0);
\draw[red, thick](-6,-6)--(0,-6);
\draw[red, thick](0,18)--(6,0);
\draw[blue, thick](-6,0)--(-6,12);
%\draw[thick, red](0, 9)--(-6,0);
\draw[red, thick](0,6)--(0,12);
\draw[blue, thick](-6,0)--(-6,-6);
\draw[blue, thick](-6,0)--(0,-6);
\draw[blue, thick](-6,0)--(0,6);
%\draw[blue, thick](-6,0)--(0,9);
\draw[blue, thick](-6,0)--(0,12);
\draw[blue, thick](-6,0)--(6,0);
\draw[red, thick](-6,12)--(0,18);
\draw[blue, thick](-6,0)--(0,18);
%\caption{Two of the $y_i$'s are distinct.}
\end{tikzpicture}
\label{$4$ triangles on an edge}
\caption{Finding a $2$-book when there are $4$ hyperedges sitting on a pair of vertices.}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55





\begin{lemma}
In a triangle in $G$ two edges are colored blue.
\end{lemma}  
\begin{proof}
Let the vertices of the triangle be $x_1,x_2$ and $x_3$.  We will deal with the different possibilities in the following cases:
\subsection*{Case $1$: There is a triangle with $3$ blue edges.}
Let $y_i$ be the third vertex of hyperedges sitting on the edge $x_ix_{i+1}$ [see Figure \ref{fig_bbb}].  The hyperedges $x_2x_3y_3, x_1x_2y_2$ and $x_1x_3y_4$ form a triangle.  The other two edges of the diamond come from the hyperedges $x_1x_3y_1$ and the hyperedge sitting on the edge $x_3y_1$.
\begin{figure}[h]
\centering
\begin{tikzpicture}[scale=0.2]
\node at (-1,-1){$x_1$};
\node at (13,-1){$x_2$};
\node at (6,7){$x_3$};
\node at (13.5,6){$y_3$};
\node at (-1,6.9){$y_1$};
\node at (6,-7){$y_2$};
\node at (-4.5,9){$y_4$};
\draw[blue, thick](6,6)--(12,6);
\draw[blue, thick](6,6)--(0,6);
\draw[red, thick](0,6)--(0,0);
\draw[blue, thick](0,0)--(6,-6);
\draw[red, thick](6,-6)--(12,0);
\draw[red, thick](12,0)--(12,6);
\draw[red, thick](0,0)--(-3,9);
\draw[blue, thick](-3,9)--(6,6);
\draw[blue, thick](12,0)--(6,6);
\draw[blue, thick](12,0)--(0,0);
\draw[blue, thick](0,0)--(6,6);
\draw[fill=black](0,0)circle(9pt);
\draw[fill=black](12,0)circle(9pt);
\draw[fill=black](6,6)circle(9pt);
\draw[fill=black](0,6)circle(9pt);
\draw[fill=black](12,6)circle(9pt);
\draw[fill=black](-3,9)circle(9pt);
\draw[fill=black](6,-6)circle(9pt);
\end{tikzpicture}

\caption{The different possibilities with a triangle having three blue edges.}
\label{fig_bbb}
\end{figure}

\subsection*{Case $2$: There is a triangle with $3$ red edges.}
We have three possibilities depending on whether the third vertex of the hyperedge sitting on $x_ix_{i+1}$ is distinct or not, as shown in the following Figures \ref{fig_rrr}.  In each case we can find a diamond.  For example, when all the $y_i$'s are distinct.  The hyperedges $x_1y_2x_3, x_2y_3x_3$ and $x_3y_1x_1$ form a triangle.  The two other of the diamond is formed by the hyperedges sitting on the edge $x_3y_3$ and $x_2y_3$.
\begin{figure}[h]
\centering
\begin{tikzpicture}[scale=0.2]
\draw[fill=black](0,0)circle(3pt);
\draw[fill=black](12,0)circle(3pt);
\draw[fill=black](6,6)circle(3pt);
\draw[fill=black](0,6)circle(3pt);
\draw[fill=black](12,6)circle(3pt);
\node at (-1,-1){$x_1$};
\node at (12,-2){$x_2$};
\node at (6,7){$x_3$};
\node at (13,6){$y_3$};
\node at (-1,6){$y_1$};
\node at (6,-7){$y_2$};


\draw[blue, thick](6,6)--(12,6);
\draw[blue, thick](6,6)--(0,6);
\draw[blue, thick](0,6)--(0,0);
\draw[blue, thick](0,0)--(6,-6);
\draw[blue, thick](6,-6)--(12,0);
\draw[blue, thick](12,0)--(12,6);
\draw[red, thick](12,0)--(6,6);
\draw[red, thick](12,0)--(0,0);
\draw[red, thick](0,0)--(6,6);


\end{tikzpicture}\quad
\begin{tikzpicture}[scale=0.2]
\draw[fill=black](0,0)circle(3pt);
\draw[fill=black](12,0)circle(3pt);
\draw[fill=black](6,6)circle(3pt);
\draw[fill=black](6,12)circle(3pt);

\node at (-1,-1){$x_1$};
\node at (12,-2){$x_2$};
\node at (6,7){$x_3$};
\node at (6,13){$y_1$};
\node at (6,-7){$y_2$};

\draw[blue, thick](0,0)--(6,12);
\draw[blue, thick](6,12)--(12,0);
\draw[blue, thick](6,12)--(6,6);
\draw[blue, thick](0,0)--(6,-6);
\draw[blue, thick](6,-6)--(12,0);
\draw[red, thick](12,0)--(6,6);
\draw[red, thick](12,0)--(0,0);
\draw[red, thick](0,0)--(6,6);


\end{tikzpicture}\quad

\begin{tikzpicture}[scale=0.2]
\draw[fill=black](0,0)circle(3pt);
\draw[fill=black](12,0)circle(3pt);
\draw[fill=black](6,6)circle(3pt);
\draw[fill=black](6,12)circle(3pt);

\node at (-1,-1){$x_1$};
\node at (12,-1){$x_2$};
\node at (6,7){$x_3$};
\node at (6,13){$y_1$};

\draw[blue, thick](0,0)--(6,12);
\draw[blue, thick](6,12)--(12,0);
\draw[blue, thick](6,12)--(6,6);

\draw[red, thick](12,0)--(6,6);
\draw[red, thick](12,0)--(0,0);
\draw[red, thick](0,0)--(6,6);


\end{tikzpicture}
\caption{The different possibilities with a triangle having three red edges.}
\label{fig_rrr}
\end{figure}
\subsection*{Case $3$: There is a triangle with $2$ red edges.}
We again have $3$ possibilities and in each case we can find a diamond.  For example, consider the second figure in Figure \ref{figure_rrb}.  The hyperedges $x_2x_3y_4, x_1x_2y_2$ and $x_1x_3y_4$ form a triangle.  The two other hyperedges are formed by $x_1x_3y_1$ and the triangle sitting on the edge $x_3y_1$.
\begin{figure}[h]
\centering
\begin{tikzpicture}[scale=0.2]
\draw[fill=black](0,0)circle(3pt);
\draw[fill=black](12,0)circle(3pt);
\draw[fill=black](6,6)circle(3pt);
\draw[fill=black](0,6)circle(3pt);
\draw[fill=black](12,6)circle(3pt);
\draw[fill=black](-3,12)circle(3pt);
\draw[fill=black](6,-6)circle(3pt);


\node at (-1,-1){$x_1$};
\node at (12,-2){$x_2$};
\node at (6,7){$x_3$};
\node at (13,6){$y_3$};
\node at (0,7){$y_1$};
\node at (6,-7){$y_2$};
\node at (-4,12){$y_4$};



\draw[blue, thick](6,6)--(12,6);
\draw[red, thick](6,6)--(0,6);
\draw[blue, thick](0,6)--(0,0);
\draw[blue, thick](0,0)--(6,-6);
\draw[blue, thick](6,-6)--(12,0);
\draw[blue, thick](12,0)--(12,6);
\draw[red, thick](12,0)--(6,6);
\draw[red, thick](12,0)--(0,0);
\draw[blue, thick](0,0)--(6,6);
\draw[blue, thick](0,0)--(-3,12);
\draw[red, thick](-3,12)--(6,6);
\end{tikzpicture}

\begin{tikzpicture}[scale=0.2]
\draw[fill=black](0,0)circle(3pt);
\draw[fill=black](12,0)circle(3pt);
\draw[fill=black](6,6)circle(3pt);
\draw[fill=black](0,6)circle(3pt);
%\draw[fill=black](12,6)circle(3pt);
%\draw[fill=black](6,12)circle(3pt);
\draw[fill=black](6,-6)circle(3pt);

\node at (-1,-1){$x_1$};
\node at (12,-2){$x_2$};
\node at (6,7){$x_3$};
%\node at (13,6){$y_3$};
\node at (0,7){$y_1$};
\node at (6,-7){$y_2$};
\node at (6,13){$y_4$};



%\draw[blue, thick](6,6)--(12,6);
\draw[red, thick](6,6)--(0,6);
\draw[blue, thick](0,6)--(0,0);
\draw[blue, thick](0,0)--(6,-6);
\draw[blue, thick](6,-6)--(12,0);
\draw[blue, thick](12,0)--(6,12);
%\draw[blue, thick](12,0)--(12,6);
\draw[red, thick](12,0)--(6,6);
\draw[red, thick](12,0)--(0,0);
\draw[blue, thick](0,0)--(6,6);
\draw[red, thick](0,0)--(6,12);
\draw[blue, thick](6,12)--(6,6);
\end{tikzpicture}

\begin{tikzpicture}[scale=0.2]
\draw[fill=black](0,0)circle(3pt);
\draw[fill=black](12,0)circle(3pt);
\draw[fill=black](6,6)circle(3pt);
\draw[fill=black](0,6)circle(3pt);
%\draw[fill=black](12,6)circle(3pt);
\draw[fill=black](-3,12)circle(3pt);
\draw[fill=black](18,-3)circle(3pt);
\node at (-1,-1){$x_1$};
\node at (12,-1){$x_2$};
\node at (6,7){$x_3$};
%\node at (13,6){$y_3$};
\node at (0,7){$y_1$};
%\node at (6,-7){$y_2$};
\node at (-4,12){$y_4$};
\node at (18,-4){$y_3$};



%\draw[blue, thick](6,6)--(12,6);
\draw[red, thick](6,6)--(0,6);
\draw[blue, thick](0,6)--(0,0);
%\draw[blue, thick](0,0)--(6,-6);
%\draw[blue, thick](6,-6)--(12,0);
%\draw[blue, thick](12,0)--(12,6);
\draw[red, thick](12,0)--(6,6);
\draw[red, thick](12,0)--(0,0);
\draw[blue, thick](0,0)--(6,6);
\draw[blue, thick](0,0)--(-3,12);
\draw[red, thick](-3,12)--(6,6);
\draw[blue, thick](18,-3)--(12,0);
\draw[blue, thick](18,-3)--(6,6);
\draw[blue, thick](18,-3)--(0,0);
\end{tikzpicture}
\label{figure_rrb}
\caption{The different possibilities with a triangle having two red edges.}
\end{figure}

\end{proof}



% 
